Fabrication of Metal Air Bridges for Superconducting Circuits using Two-photon Lithography

Extraneous high frequency chip modes parasitic to superconducting quantum circuits can result in decoherence when these modes are excited. To suppress these modes, superconducting air bridges (AB) are commonly used to electrically connect ground planes together when interrupted by transmission lines. Here, we demonstrate the use of two-photon photolithography to build a supporting 3D resist structure in conjunction with a lift-off process to create AB. The resulting aluminum AB, have a superconducting transition temperature $T_{c} = 1.08$ K and exhibit good mechanical strength up to lengths of 100 $\mu$m. A measurable amount of microwave loss is observed when 35 AB were placed over a high-$Q$ Ta quarter-wave coplanar waveguide resonator.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
